Nonlocality-Reinforced Convolutional Neural Networks for Image Denoising

We introduce a paradigm for nonlocal sparsity reinforced deep convolutional neural network denoising. It is a combination of a local multiscale denoising by a convolutional neural network (CNN) based denoiser and a nonlocal denoising based on a nonlocal filter (NLF) exploiting the mutual similarities between groups of patches. CNN models are leveraged with noise levels that progressively decrease at every iteration of our framework, while their output is regularized by a nonlocal prior implicit within the NLF. Unlike complicated neural networks that embed the nonlocality prior within the layers of the network, our framework is modular, it uses standard pre-trained CNNs together with standard nonlocal filters. An instance of the proposed framework, called NN3D, is evaluated over large grayscale image datasets showing state-of-the-art performance.

==> table/bm_experiments.tex <==
\pgfplotstableset{create on use/method/.style={create col/set list={dncnn,ffdnet,wdncnn}}}
\pgfplotstableset{create on use/source/.style={create col/set list={$z$, $\tilde{y}^{HT}_{BM3D}$, $\tilde{y}_1$}}}

\pgfplotstableread{data/urban100_dncnn_sigma75_bm_experiments_mean.csv}\fulltabletmp
\pgfplotstablevertcat{\fulltabletmp}{data/urban100_ffdnet_sigma75_bm_experiments_mean.csv}
\pgfplotstablevertcat{\fulltabletmp}{data/urban100_wdncnn_sigma75_bm_experiments_mean.csv}

\pgfplotstabletranspose[
string type,
colnames from=method,
% input colnames to=source,
columns={method, z, bm3dht,cnnf},
]{\fulltable}{\fulltabletmp}

\pgfplotstabletypeset[
print sign,
columns/source/.style={string type,column name=Source},
columns/dncnn/.style={column name=\thingcombo{DnCNN},},
columns/ffdnet/.style={column name=\thingcombo{FFDNet},},
columns/wdncnn/.style={column name=\thingcombo{\wavdncnn},},
columns={source,dncnn,ffdnet,wdncnn}
]{\fulltable}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../gse-cnn"
%%% End:


==> table/performance_ssim.tex <==
% This code assumes the following pgfplotstable keys:
% colsep=comma

\newcommand{\thingsuffix}{NLP}

\pgfplotstableread{data/ssim_set12.csv}\ssimsettwelve
\pgfplotstableread{data/ssim_bsd68.csv}\ssimbsdsixtyeight
\pgfplotstableread{data/ssim_urban100.csv}\ssimurbanhundred

\pgfplotstablevertcat{\fulltable}{\ssimsettwelve}
\pgfplotstablevertcat{\fulltable}{\ssimbsdsixtyeight}
\pgfplotstablevertcat{\fulltable}{\ssimurbanhundred}

\pgfplotstabletypeset[
        precision=4,
	create on use/dataset/.style={create col/set list={Set12,,,BSD68,,,Urban100,,}},
	columns/dataset/.style={
		string type,
		column name=Dataset,
		% Use multirow for the datasets.
		assign cell content/.code={
			\pgfmathparse{int(Mod(\pgfplotstablerow, 3))}%
			\ifnum\pgfmathresult=0%
				\pgfkeyssetvalue{/pgfplots/table/@cell content}
				{\multirow{3}{*}{\emph{##1}}}%
			\else
				\pgfkeyssetvalue{/pgfplots/table/@cell content}{}%
			\fi
		},
	},
	% This can make certain cells bold. Second form takes column names.
	%every row no 0 column no 0/.style={postproc cell content/.style={@cell content=\textbf{##1}}},
	%every row 0 column vdsr/.style={postproc cell content/.style={@cell content=\textbf{##1}}},
	% Add a midrule after every dataset.
	every nth row={3}{before row=\midrule},
	columns/sigma/.style={column name=$\sigma$, precision=0},
	columns/bm3d/.style={column name=BM3D},
	columns/dncnn/.style={column name=DnCNN},
	columns/dncnnnlp/.style={column name=DnCNN-\thingsuffix},
	columns/ffdnet/.style={column name=FFDNet},
	columns/ffndetnlp/.style={column name=FFDNet-\thingsuffix},
	columns/cnn/.style={column name=CNN},
	columns/cnnnlp/.style={column name=CNN-\thingsuffix},
	columns={dataset, sigma, bm3d, dncnn, dncnnnlp, ffdnet, ffdnetnlp, cnn, cnnnlp},
]{\fulltable}

